Interdependent Values without Single-Crossing

We consider a setting where an auctioneer sells a single item to $n$ potential agents with {\em interdependent values}. That is, each agent has her own private signal, and the valuation of each agent is a known function of all $n$ private signals. This captures settings such as valuations for artwork, oil drilling rights, broadcast rights, and many more. In the interdependent value setting, all previous work has assumed a so-called {\sl single-crossing condition}. Single-crossing means that the impact of agent $i$'s private signal, $s_i$, on her own valuation is greater than the impact of $s_i$ on the valuation of any other agent. It is known that without the single-crossing condition an efficient outcome cannot be obtained. We study welfare maximization for interdependent valuations through the lens of approximation. We show that, in general, without the single-crossing condition, one cannot hope to approximate the optimal social welfare any better than the approximation given by assigning the item to a random bidder. Consequently, we introduce a relaxed version of single-crossing, {\sl $c$-single-crossing}, parameterized by $c\geq 1$, which means that the impact of $s_i$ on the valuation of agent $i$ is at least $1/c$ times the impact of $s_i$ on the valuation of any other agent ($c=1$ is single-crossing). Using this parameterized notion, we obtain a host of positive results. We propose a prior-free deterministic mechanism that gives an $(n-1)c$-approximation guarantee to welfare. We then show that a random version of the proposed mechanism gives a prior-free universally truthful $2c$-approximation to the optimal welfare for any concave $c$-single crossing setting (and a $2\sqrt{n}c^{3/2}$-approximation in the absence of concavity). We extend this mechanism to a universally truthful mechanism that gives $O(c^2)$-approximation to the optimal revenue.

==> supercLBApp.tex <==
\subsection{No $c$-approximation exists for more than $2$ agents with more than $2$ signals}\label{sec:nocapprox}

%Here we prove the following proposition from Section~\ref{sec:warmups}.

The smallest possible case beyond where we know we have a tight $c$-approximation---either with more than two bidders, or with $n$ bidders with signal space of size more than $2$---is to have three bidders, two with signal space of size 2, and one with signal space of size 3.  That is, $S_2 = S_3 = \{0,1\}$ and $S_1 = \{0,1,2\}$.

\begin{numberedproposition}{\ref{prop:superc}}
Let $n$ be the number of bidders, $k_i$ the size of bidder $i$'s signal space, and $k = \max_i k_i$.  For any setting where $n \geq 3$, $k_i \geq 3$ for some $i$, and the buyer valuations satisfy $c$-single-crossing, there exists an instance where no truthful deterministic prior-free allocation can achieve a $c$-approximation to welfare. 
\end{numberedproposition}

In Figure~\ref{fig:nocapxconstraints}, we describe a structure of the valuations where the signal space is $S_1\times S_2 \times S_3=\{0,1,2\}\times\{0,1\}\times\{0,1\}$. In this structure, we show that in order to have a $c$-approximation to the welfare, a number of constraints on the allocation must be satisfied, and combining these constraints yields a contradiction. numbers that support his structure are depicted in Appendix \ref{sec:nocapproxnumbers}.

Consider the structure depicted in Figure~\ref{fig:nocapxconstraints}. At valuation profile $(s_1=2,s_2=0,s_3=0)$, no bidder has a value that $c$-approximates bidder~2's value.

, in order to have a $c$-approximate allocation, they will impose a number of constraints on the allocation.  
 
  In Figure~\ref{fig:nocapxconstraints}, we describe the general structure of the valuations such that, in order to have a $c$-approximate allocation, they will impose a number of constraints on the allocation.  One can verify there are numbers that support this structure using a computer program, which are listed below.
  %We include precise valuations that satisfy $c$-single crossing for $c=2$ that satisfy these constraints in~\ref{sec:precisenumbers}.

\begin{figure}[h!]
%\includegraphics[scale=.35]{images/nocapxslice0constraints} \quad\quad\quad \includegraphics[scale=.35]{images/nocapxslice1constraints}
\includegraphics[scale=.35]{images-new/figure6-left} \quad\quad\quad \includegraphics[scale=.35]{images-new/figure6-right}
\caption{Left: The constraints on approximation of the values in the slice where $s_3 = 0$.  Right: The constraints where $s_3 = 1$.  The labeling ``Not $i$" indicates that $i$ cannot win the item and give a $c$-approximation.  The labeling ``Must be $i$" indicates that no other bidder could win the item and give a $c$-approximation.}
\label{fig:nocapxconstraints}
\end{figure}

\begin{figure}[h!]
%\includegraphics[scale=.3]{images/nocapxslice0colored}  \quad\quad \quad
%\includegraphics[scale=.3]{images/nocapxslice1colored} %\quad\quad\quad \includegraphics[scale=.3]{images/nocapx3dnewprop}
\includegraphics[scale=.3]{images-new/figure7-left}  \quad\quad \quad \includegraphics[scale=.3]{images-new/figure7-right} 
\caption{The implications of the valuations on the allocation rule in order to have a $c$-approximation, which leads to a propagation conflict at profile $(1,1,1)$ where both $1$ and $3$ have been propagated as the winners.} % Bottom: A three-dimensional illustration of the propagations and conflict.}
\label{fig:noxapxcolored}
\end{figure}

As depicted in Figure~\ref{fig:noxapxcolored}, the valuations gives us no choice about the allocation in the slice where $s_3 = 0$; the allocation at every profile is uniquely determined either by approximation (to have a $c$-approximation), by propagation, or by avoiding propagation conflicts.  Then, in the slice where $s_3 = 1$, the only allocation we can have in order to have a $c$-approximation results in a conflict, showing that there does not exist a monotone allocation that gives a $c$-approximation under this valuation profile.  Hence, we cannot hope for a $c$-approximation when we have more than two bidders and more than 2 signals in the signal space of any bidder.

\subsubsection{Precise Numbers} \label{sec:precisenumbers}

In this example, $c = .2757$.

\begin{tabular}{| c | c | c |} \hline
$(0,1,0)$ & $(1,1,0)$ & $(2,1,0)$ \\
$v_1 = 0.00722 $ & $v_1 = 0.01453$ & $v_1 = 0.01781$ \\
$v_2 = 0.00429$ & $v_2 = 0.00809$ & $v_2 = 0.01465$ \\
$v_3 = 0.00318$ & $v_3 = 0.01780$ & $v_3 = 0.01781$ \\ \hline
$(0,0,0)$ & $(1,0,0)$ & $(2,0,0)$ \\
$v_1 = 0$ & $v_1 = 0.00010$ & $v_1 = 0.00338$ \\
$v_2 = 0.67604$ & $v_2 = 0.00087$ & $v_2 = 0.00744$ \\
$v_3 = 0.00317$ & $v_3 = 0.00337$ & $v_3 = 0.00338$ \\ \hline
\end{tabular} \quad \quad \quad
\vspace{.5cm}
\begin{tabular}{| c | c | c |} \hline
$(0,1,1)$ & $(1,1,1)$ & $(2,1,1)$ \\
$v_1 = 0.00945$ & $v_1 = 0.01676$ & $v_1 = 0.02004$ \\
$v_2 = 0.00430$ & $v_2 = 0.00810$ & $v_2 = 0.01466$ \\
$v_3 = 0.00430$ & $v_3 = 0.01891$ & $v_3 = 0.01892$ \\ \hline
$(0,0,1)$ & $(1,0,1)$ & $(2,0,1)$ \\
$v_1 = 0.00223$ & $v_1 = 0.00233$ & $v_1 =  0.00561$ \\
$v_2 = 0.00069$ & $v_2 = 0.00089$ & $v_2 = 0.00745$ \\
$v_3 = 0.00428$ & $v_3 = 0.00449$ & $v_3 = 0.00450$ \\ \hline
\end{tabular}


